FlexRDZ: Autonomous Mobility Management for Radio Dynamic Zones

FlexRDZ is an online, autonomous manager for radio dynamic zones (RDZ) that seeks to enable the safe operation of RDZs through real-time control of deployed test transmitters. FlexRDZ leverages Hierarchical Task Networks and digital twin modeling to plan and resolve RDZ violations in near real-time. We prototype FlexRDZ with GTPyhop and the Terrain Integrated Rough Earth Model (TIREM). We deploy and evaluate FlexRDZ within a simulated version of the Salt Lake City POWDER testbed, a potential urban RDZ environment. Our simulations show that FlexRDZ enables up to a 20 dBm reduction in mobile interference and a significant reduction in the total power of leaked transmissions while preserving the overall communication capabilities and uptime of test transmitters. To our knowledge, FlexRDZ is the first autonomous system for RDZ management.

==> discussion.tex <==
\section{Discussion and Limitations}
\label{sec:discussion}

{\bf Scalability.} The computational complexity of simulating an RDZ grows extremely fast relative to the number of deployed test transmitter; however, we argue that this is not an immediate concern for \Tool{}. % and the level of dynamicity of the environment, making robust evaluations difficult. 
First, our evaluation only needs to consider a small number of transmitters. In contrast to non-urban RDZs, the size of an urban RDZ is substantially limited by the amount of available area within the urban environment. Furthermore, only a subset of operating parameters may be compliant with the regulations associated with an urban RDZ, limiting the number of potential users even more. Finally, since RDZs are access-based environments, only a subset of users may be eligible to deploy their test transmitters at any given time. Thus, our evaluation only needs to consider a small number of mobile transmitters. building infrastructure to enable large-scale evaluations is an area of future research.

% , e.g.,\ consider the difference in scale between a non-urban deployment in the desert of New Mexico and an urban deployment in the POWDER campus. As a result, the limited area will constrain the number of test transmitters deployed.  , further reducing the number of deployed devices. ; however, 


{\bf Online Modeling.} The current version of \Tool{} leverages a static digital twin of the RDZ, with a majority of the environment information being loaded and processed during initialization. However, a static digital twin model fails to accurately model more dynamic scenarios (e.g.,\ sharp changes in weather), leading to divergence from reality and misinforming \Tool{}'s planning decisions. To ensure that \Tool{}'s digital twin accurately reflects reality, enabling the ability to update the internal propagation model's parameters based on environmental updates in an online manner may be an area of future research.


{\bf Real World Deployment.} Although we simulate an urban RDZ in the downtown Salt Lake City area with real parameters from the POWDER testbed, our simulations and datasets are limited. In a real RDZ deployment, many outside factors exist that cannot be controlled and severely affect management and modeling, e.g., weather, number of outside users in the vicinity, and control delay. Thus, to truly benchmark our system, we must move to a real environment. We leave this as an area of future research.
